Magic123: One Image to High-Quality 3D Object Generation Using Both 2D and 3D Diffusion Priors

We present Magic123, a two-stage coarse-to-fine approach for high-quality, textured 3D meshes generation from a single unposed image in the wild using both2D and 3D priors. In the first stage, we optimize a neural radiance field to produce a coarse geometry. In the second stage, we adopt a memory-efficient differentiable mesh representation to yield a high-resolution mesh with a visually appealing texture. In both stages, the 3D content is learned through reference view supervision and novel views guided by a combination of 2D and 3D diffusion priors. We introduce a single trade-off parameter between the 2D and 3D priors to control exploration (more imaginative) and exploitation (more precise) of the generated geometry. Additionally, we employ textual inversion and monocular depth regularization to encourage consistent appearances across views and to prevent degenerate solutions, respectively. Magic123 demonstrates a significant improvement over previous image-to-3D techniques, as validated through extensive experiments on synthetic benchmarks and diverse real-world images. Our code, models, and generated 3D assets are available at https://github.com/guochengqian/Magic123.

==> figures/combined_dataset.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.49\textwidth]{figures/src/input_nerf_dataset.png} \includegraphics[trim={0 0 6.2cm 1.6cm},clip,width=0.49\textwidth]{figures/src/input_realfusion_dataset.png}
\caption{Sample images from NeRF4 dataset (\textit{left}) and RealFusion15 dataset (\textit{right}).}
\label{fig:combined_dataset}
\end{figure}


==> figures/input_nerf4.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=0.8\textwidth]{figures/src/input_nerf_dataset.png}
\caption{Input images from NeRF4 dataset.}
\label{fig:nerf4_dataset}
\end{figure}


==> figures/input_realfusion15.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=0.9\textwidth]{figures/src/input_realfusion_dataset.png}
\caption{Input images from RealFusion15 dataset.}
\label{fig:realfusion15_dataset}
\end{figure}


==> sections/checklist.tex <==

\newpage

\section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{All claims all accurately reflect the paper's contributions, and were validated in the \seclabel~\ref{sec:ablation}. }
  \item Did you describe the limitations of your work?
    \answerYes{The limitation was discussed at \seclabel~\ref{sec:limit}.} 
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{Available in the \supp.} 
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{Our paper conforms to the ethics review guidelines.}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Available in the \supp.}
  \item Did you specify all the training details (\eg data splits, hyperparameters, how they were chosen)?
    \answerYes{See \seclabel~\ref{sec:exp} Experimental setups for optimization techniques and \seclabel~\ref{sec:ablation_train_strategies} for data augmentations used in training.}
	\item Did you report error bars (\eg with respect to the random seed after running experiments multiple times)?
    \answerYes{We reported all results with average and standard deviation in three random runs except the S3DIS 6-fold. We trained on all areas for three times, and picked the best on validation for each area, then performed the 6-fold cross-validation. Note that the averaged results with error bars on S3DIS area 5 are available in \tablabel~\ref{tab:ablate_s3dis} and \supp.}
	\item Did you include the total amount of compute and the type of resources used (\eg type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See \seclabel~\ref{sec:exp} Experimental setups.}
\end{enumerate}

\item If you are using existing assets (\eg code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We cited.}
  \item Did you mention the license of the assets?
    \answerNo{All of the code, models, and datasets we used are publicly available.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{We included our code and models in \supp.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{All the data is publicly available. }
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}



==> sections/preliminary.tex <==
\section{Preliminary}\label{sec:prelinminary}
% \todo{remove this part if no space}

% \inlinesection{Neural radiance fields (NeRFs)}
A neural radiance field (NeRF)~\cite{NeRF, NeuralVolumes} is a neural network-based representation of a 3D volume's radiance field, optimized through differentiable volumetric rendering~\cite{VolumeRenderingDigest} from multiple posed views.
A pixel's (RGB) color $C(\ray) \in \Rr^3$ for the ray $\ray(t) = \rayo + t \raydir$ with origin $\bm o \in \Rr^3$, direction $\bm d \in \Ss^2$, and boundaries $t \in [t_n, t_f] \subseteq \Rr_+$, is an integrated color value $\bm c(\ray(t), \raydir) \in \Rr^3$ along the ray~\cite{NeRF}:
\begin{equation}\label{eq:nerf}
C(\ray) = \int_{t_n}^{t_f} \bm{c}(\ray(t), \raydir) T(t) \sigma(\ray(t)) \text{d}t,
\end{equation}
where $\sigma(t) \in \Rr_+$ is the volume density.
Both color $\bm c$ and density $\sigma(t)$ are predicted by the neural network, which is typically constructed by MLPs.
$T(t) \in [0, 1]$ is the accumulated transmittance:
\begin{equation}\label{eq:acc-transmittance}
T(t) = \exp \left(-\int_{t_n}^{t_f} \sigma(\mathbf{r}(s)) \text{d} s \right).
\end{equation}

Recently, there appeared numerous works that adopted faster grid-based representations \cite{PlenOctrees, plenoxels, KiloNeRF, InstantNGP, NSVF, EG3D}.
Instant-NGP~\cite{InstantNGP} is the most popular accelerated NeRF to date and has thus been adopted in our pipeline as the efficient NeRF backbone. 


==> tables/ablate_noise.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[t]
\centering
\caption{Ablation study on the selection of noise range for the NeRF4 dataset.}
\label{tab:ablate_noise}
\resizebox{0.6\textwidth}{!}{%
\begin{tabular}{@{}ccccccc@{}}
\toprule
\textbf{Noise} & \textbf{{[}0.02, 0.6{]}} & \textbf{{[}0.1,0.6{]}} 
&\textbf{{[}0.2,0.6{]}}
& \textbf{{[}0.2,0.8{]}} & \textbf{{[}0.2,0.98{]}} & \textbf{{[}0.4,0.6{]}} \\ \midrule
\textbf{CLIP-Similarity$\uparrow$} & 0.8  & 0.8  & 0.8& 0.8  & 0.8  & 0.8  \\
\textbf{PSNR$\uparrow$}            & 24.1 & 22.5 & 23.0 & 24.0 & 23.6 & 23.7 \\
\textbf{LPIPS$\downarrow$}           & 0.04  & 0.05  & 0.05 & 0.04  & 0.04  & 0.04  \\ \bottomrule
\end{tabular}%
}
\end{table}

==> tables/ablate_resolution.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[t]
\centering
\caption{Ablation study on the resolution of the coarse stage for the NeRF4 dataset.}
\label{tab:ablate_resolution}
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{@{}ccccc@{}}
\toprule
\textbf{Resolution}                & \textbf{32} & \textbf{64} & \textbf{128} & \textbf{256} \\ \midrule
\textbf{CLIP-Similarity$\uparrow$} & 0.7        & 0.8        & 0.8        & \textbf{0.8}         \\
\textbf{PSNR$\uparrow$}            & 20.49       & 22.32       & 22.97       & \textbf{24.22}        \\
\textbf{LPIPS$\downarrow$}           & 0.11        & 0.07        & 0.05        & \textbf{0.03}         \\ \bottomrule
\end{tabular}%
}
\end{table}

==> tables/ablation_2d-3d-coarse-fine.tex <==

\begin{table}[t]
\centering
\caption{Quantitative comparisons of the coarse and fine stages between Magic123 with only 2D prior ($\lambda_{2D}$=$1$,$=\lambda_{3D}$=$0$), Magic123 with only 3D prior $\lambda_{2D}$=$0$,$\lambda_{3D}$=$40$, and Magic123 ($\lambda_{2D}$=$1$,$\lambda_{3D}$=$40$)
% \todo{@wayne update table, value comment below}
}
\label{tab:2d-3d-coarse-fine}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}c|cccccccc@{}}
\toprule
\textbf{Dataset} & \textbf{Metrics\textbackslash{}Methods} 
& 2D prior (Coarse) & 2D prior & 3D prior (Coarse) & 3D  prior & Magic123 Coarse & \textbf{Magic123}  \\ \midrule
\multirow{3}{*}{\textbf{NeRF4}}        
& CLIP-Similarity$\uparrow$  & 0.60 & 0.67 & 0.62 & 0.71 & 0.68  & \textbf{0.80} \\
& PSNR$\uparrow$             & 24.11 & 24.58 & 23.96 & 24.69 & 23.67  & \textbf{24.62} \\
& LPIPS$\downarrow$           & 0.04 & 0.03 & 0.05 & 0.03 & 0.05  & \textbf{0.03} \\ \midrule
\multirow{3}{*}{\textbf{RealFusion15}} 
& CLIP-Similarity$\uparrow$ & 0.77 & 0.78 & 0.75 & 0.76 & 0.79  & \textbf{0.82} \\
& PSNR$\uparrow$            & 19.77 & 19.60 & 19.49 & 19.58 & 19.42  & \textbf{19.50} \\
& LPIPS$\downarrow$          & 0.10 & 0.09 & 0.11 & 0.10 & 0.11  & \textbf{0.10} \\ \bottomrule
\end{tabular}
}
\end{table}

==> tables/result_natural.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[!htb]
\caption{Object-wise results on RealFusion15 dataset.}
\label{tab:natural}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}l|cccc|cccc|cccc@{}}
\toprule
Metrics                   & \multicolumn{4}{c|}{\textbf{CLIP-similarity$\uparrow$}}    & \multicolumn{4}{c|}{\textbf{PSNR$\uparrow$}}                & \multicolumn{4}{c}{\textbf{LPIPS$\downarrow$}}               \\ \midrule
Objects                   & NeuralLift & 3DFuse & RealFusion & \textbf{Ours} & NeuralLift & 3DFuse & RealFusion & \textbf{Ours}  & NeuralLift & 3DFuse & RealFusion & \textbf{Ours} \\ \midrule
\textit{banana}           & 0.68       & 0.78   & \textbf{0.83}       & 0.81 & 12.82      & 13.04  & 18.21      & \textbf{18.60} & 0.33       & 0.33   & \textbf{0.12}       & 0.15 \\
\textit{blue bird}             & 0.78       & 0.71   & 0.82       & \textbf{0.87} & 12.40      & 9.73   & 19.53      & \textbf{19.79} & 0.23       & 0.29   & 0.08       & \textbf{0.07} \\
\textit{bird sparrow}     & 0.71       & 0.61   & 0.70       & \textbf{0.82} & 11.01      & 10.96  & \textbf{18.74}      & 17.78 & 0.28       & 0.29   & 0.09       & \textbf{0.07} \\
\textit{cactus}           & 0.73       & 0.76   & 0.69       & \textbf{0.80} & 12.23      & 12.14  & \textbf{18.14}      & 17.73 & 0.26       & 0.25   & \textbf{0.12}       & 0.15 \\
\textit{cake}             & 0.56       & 0.62   & 0.71       & \textbf{0.76} & 10.44      & 10.11  & 17.42      & \textbf{17.64} & 0.75       & 0.44   & \textbf{0.14}       & 0.15 \\
\textit{cat statue}       & 0.63       & 0.59   & 0.64       & \textbf{0.77} & 9.97       & 9.15   & \textbf{18.61}      & 17.88 & 0.38       & 0.43   & 0.12       & \textbf{0.09} \\
\textit{cherry}           & 0.75       & 0.80   & 0.64       & \textbf{0.81} & 10.45      & 11.39  & \textbf{19.40}      & 18.50 & 0.36       & 0.25   & 0.25       & \textbf{0.06} \\
\textit{colorful teapot}  & 0.55       & 0.56   & 0.63       & \textbf{0.64} & 10.17      & 10.94  & 21.34      & \textbf{30.09} & 0.33       & 0.32   & 0.16       & \textbf{0.03} \\
\textit{donut}            & 0.79       & \textbf{0.81}   & 0.63       & 0.74 & 14.00      & 13.17  & 19.87      & \textbf{20.82} & 0.31       & 0.29   & 0.13       & \textbf{0.10} \\
\textit{metal dragon statue}  & 0.61       & 0.61   & 0.66       & \textbf{0.75} & 9.42       & 8.98   & \textbf{17.26}      & 16.40 & 0.39       & 0.43   & \textbf{0.14}       & 0.17 \\
\textit{stone dragon statue}  & 0.63       & 0.65   & 0.65       & \textbf{0.78} & 11.72      & 8.81   & 16.66      & \textbf{17.48} & 0.40       & 0.42   & 0.20       & \textbf{0.16} \\
\textit{fish nemo}        & 0.59       & 0.73   & 0.79       & \textbf{0.89} & 7.95       & 9.56   & 22.88      & \textbf{24.94} & 0.73       & 0.39   & 0.10       & \textbf{0.03} \\
\textit{watercolor horse} & 0.62       & 0.57   & 0.69       & \textbf{0.77} & 8.74       & 6.78   & \textbf{17.08}      & 16.10 & 0.51       & 0.90   & 0.16       & \textbf{0.11} \\
\textit{microphone}       & 0.65       & 0.70   & 0.46       & \textbf{0.82} & 16.42      & 11.77  & 21.85      & \textbf{22.81} & 0.14       & 0.22   & 0.09       & \textbf{0.04} \\
\textit{teddy bear}       & 0.50       & 0.52   & 0.54       & \textbf{0.72} & 8.49       & 8.33   & \textbf{16.10}      & 15.17 & 0.41       & 0.40   & 0.15       & \textbf{0.11} \\ \midrule
\textbf{Average}                   & 0.65       & 0.67   & 0.67       & \textbf{0.78} & 11.08      & 10.32  & 18.87      & \textbf{19.45} & 0.39       & 0.38   & 0.14       & \textbf{0.10} \\
\bottomrule
\end{tabular}%
}
\end{table}

==> tables/result_nerf.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[!htb]
\caption{Object-wise results on NeRF4 dataset.}
\label{tab:nerf}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}l|cccc|cccc|cccc@{}}
\toprule
Metrics        & \multicolumn{4}{c|}{\textbf{CLIP-similarity$\uparrow$}}    & \multicolumn{4}{c|}{\textbf{PSNR$\uparrow$}}       & \multicolumn{4}{c}{\textbf{LPIPS$\downarrow$}}      \\ \midrule
Objects        & NeuralLift & 3DFuse & RealFusion & \textbf{Ours} & NeuralLift & 3DFuse & RealFusion & \textbf{Ours}  & NeuralLift & 3DFuse & RealFusion & \textbf{Ours} \\ \midrule
\textit{chair} & 0.59       & 0.57   & 0.36       & \textbf{0.76} & 16.95      & 14.37  & 18.99      & \textbf{30.35} & 0.23       & 0.20   & 0.15       & \textbf{0.02} \\
\textit{drums} & 0.60       & 0.71   & 0.45       & \textbf{0.81} & 10.26      & 7.49   & 13.52      & \textbf{19.49} & 0.47       & 0.47   & 0.31       & \textbf{0.07} \\
\textit{ficus} & 0.38       & 0.47   & 0.28       & \textbf{0.65} & 11.72      & 14.16  & 16.28      & \textbf{21.06} & 0.60       & 0.20   & 0.25       & \textbf{0.05} \\
\textit{mic}   & 0.50       & 0.64   & 0.42       & \textbf{0.81} & 11.27      & 10.56  & 12.68      & \textbf{20.98} & 0.30       & 0.30   & 0.26       & \textbf{0.05} \\ \midrule
\textbf{Average}        & 0.52       & 0.60   & 0.38       & \textbf{0.75} & 12.55      & 11.64  & 15.37      & \textbf{22.97} & 0.40       & 0.29   & 0.24       &\textbf{ 0.05}
\\ \bottomrule
\end{tabular}%
}
\end{table}
